OA-MPC: Occlusion-Aware MPC for Guaranteed Safe Robot Navigation with Unseen Dynamic Obstacles

For safe navigation in dynamic uncertain environments, robotic systems rely on the perception and prediction of other agents. Particularly, in occluded areas where cameras and LiDAR give no data, the robot must be able to reason about potential movements of invisible dynamic agents. This work presents a provably safe motion planning scheme for real-time navigation in an a priori unmapped environment, where occluded dynamic agents are present. Safety guarantees are provided based on reachability analysis. Forward reachable sets associated with potential occluded agents, such as pedestrians, are computed and incorporated into planning. An iterative optimization-based planner is presented that alternates between two optimizations: nonlinear Model Predictive Control (NMPC) and collision avoidance. Recursive feasibility of the MPC is guaranteed by introducing a terminal stopping constraint. The effectiveness of the proposed algorithm is demonstrated through simulation studies and hardware experiments with a TurtleBot robot. A video of experimental results is available at \url{https://youtu.be/OUnkB5Feyuk}.

==> SEC2_OLD.tex <==
\section{Related work}
\label{SEC2}
% Reachability analysis is a powerful set of theoretical tools to analyze safety-critical systems. They have been extensively studied and widely used to achieve safety guarantees \cite{Gillula2010, Fisac2015}.
% To perform reachability analysis set-based approaches or Hamilton-Jabobian (HJ) reachability are employed. While set-based approaches are limited to linear dynamics and therefore cannot provide exact reachability for nonlinear systems, Hamilton-Jabobian partial differential equations (PDEs) can handle nonlinear dynamics. However, HJ reachability scales poorly with state dimension and is computationally expensive. Thus, there is a trade-off between providing safety guarantees and computational efficiency and stronger guarantees can be provided with higher computational cost.  
Hamilton-Jabobian (HJ) reachability is a standard method to analyze safety, but it is computationally expensive.
In particular, for real-time applications such as robot navigation, to address this challenge and reduce the online computation burden, the authors in 
% \cite{Dabadie2014, Ding2010}, and
\cite{Ding2011} propose precomputation of HJ reachable sets offline and storing them in a look-up table to be used online. In \cite{Herbert2017}, the authors present a fast and safe tracking approach (FaSTrack) in which slow offline computation provides safety guarantees for a faster online planner.
% FaSTrack includes a complex offline tracking system and a simplified online planning system. A pursuit-evasion game between the two systems is precomputed using HJ reachability and a safety bubble is built around the planning system. Online, based on the relative state of the two systems a safe controller is selected, using the precomputed look-up table. 
In \cite{David2018}, the authors propose to extend the FaSTrack approach to a meta-planning scheme in which a refined offline computation enables safe switching between different online planners. However, these approaches are restricted to static environments and are not applicable to dynamic environments with moving obstacles. In \cite{Zhan-RSS-21}, the authors present a pursuer-evader game theoretic framework for occlusion-aware driving (in a dynamic environment) with safety guarantees using reachability, and simulation studies are provided by assuming linear dynamics (double integrator) for the vehicle model.  

Joint active perception and planning help the robot to gather additional information about the occluded regions and gain visibility in a partially occluded environment. The authors in \cite{Falanga2018_PAMPC}, propose a perception-aware MPC framework for quadrotors that simultaneously optimizes planning and perception objectives. In \cite{Lee2020_AggressivePerceptionNavigation}, an MPC framework is coupled with a visual pipeline. A deep optical flow dynamics presented as a combination of optical flow and robot dynamics is used to predict the movement of points of interest. The proposed Pixel MPC algorithm controls the robot to accomplish a high-speed task while maintaining the visibility of the important features. In \cite{Higgins2021} a geometric heuristic is proposed to define a visibility measure around a corner. The perception objective (visibility) is added to the MPC multi-objective cost to navigate the occluded corner while maximizing visibility. In our proposed approach visibility maximization is not incorporated explicitly. However, by including a minimum safety distance to the avoid set, the robot indirectly maximizes its visibility to minimize the occluded area.

Other works including \cite{Hoerman2017_CrossroadsBlindCorners} and \cite{Lee2017_CollisionRiskAssessment},
% ,Chung2009_SafeNavigation,Brechtel2014_ProbaDecisionMaking,Miller2008_Skynet,Sadou2004_OcclusionsObstacleDetection,Bouraine2014_PassivelySafePlanning,Zhan2016_NonConservativelyDefenseStrat}
% consider the risk caused by occlusions, ranging from simple visibility modeling for pre-detected obstacles like \cite{Miller2008_Skynet}, to more complex multi-layered models proposed in \cite{Hoerman2017_CrossroadsBlindCorners}. 
These works minimize the risk of collision but they do not provide formal safety guarantees. In \cite{Andersen2017}, MPC planning is proposed in which the objective is to maximize visibility,
% or field-of-view, while safety constraints are checked by a higher-level state machine
but formal safety guarantees or recursive feasibility of MPC is not provided. Compared to these online navigation approaches, our proposed MPC provides safety guarantees by online computation of reachable sets.  

In \cite{Nager2019}, an inference and motion planning scheme is proposed to guarantee safety with respect to hypothetical hidden agents.
% that have not been observed using sensor scans.
Reachable sets are constructed by taking an occupancy map and enlarging the occluded boundaries.
% However, this work assumes the availability of a class of possible intentions for other agents which is used in the prediction step of inference to evolve the dynamics of other agents. 
Compared to this work, our approach does not make any assumptions regarding the intention of hidden agents. Our proposed framework is dynamic-agnostic with respect to hidden agents and assumes the hidden agents may move in any arbitrary direction. 

% a novel MPC-based framework to navigate occluding environments that increases visibility while considering uncertainties. Uncertainties are considered through an occupancy mapping-based approach to autonomously decide if it is safe to move around an occluding corner. If it is not safe, the policy framework chooses a motion that promotes visibility as it approaches the occlusion, thereby reducing uncertainty while navigating around a corner safer and faster.

% Therefore, some recent literature including [citation] present motion planning algorithms that integrate visibility maximization. Indeed, \cite{Penin2020_AggressiveTargetTracking}'s work aims to follow in a smooth but reactive way a moving target while avoiding obstacles in the environment and occlusions in the image space. A vision-based approach is implemented on a real quadrotor on multi-objective optimization, with an occlusion constraint formulation, keeping a target in its camera's field of view. 

% Inspired by the coordination of human eyes, the work \cite{Chang2020_CrossDroneCoordination} has explored the the visibility in multi-vehicles' frameworks. Their idea is to use distributed target measurements to overcome the occlusion effects. The approach of recognizing and supervising a geometrically complex environment by flying UAVs next to it has also been described in the \cite{Zhang2019_OcclusionAwareUAV}'s work. The work \cite{Fehr2014_OcclusionAlleviation} even equipped a robot with a sensor capable of searching for better points to view to facilitate object classification in occluded environments.

% In this context of the unknown uncertainty, \cite{Janson2018_OptimalityBenchmarks} proposes a planning trajectory when the obstacle-state is a-priori unknown. This literature considers the occlusions by static obstacles, and not dynamic ones, that could appear from behind the vehicle for example.
% Considering the behavior of other vehicles and of humans in autonomous transportation, \cite{Orzechowski2018_SetBasedSafety} calculated the reachability sets from an occluded area in order to avoid collisions. This literature takes into the consideration that all cars obey traffic laws and therefore cannot be generalized to all maps.
